Evaluation of Orientation Ambiguity and Detection Rate in April Tag and WhyCode

Fiducial systems provide a computationally cheap way for mobile robots to estimate the pose of objects, or their own pose, using just a monocular camera. However, the orientation component of the pose of fiducial markers is unreliable, which can have destructive effects in autonomous drone landing on landing pads marked with fiducial markers. This paper evaluates the April Tag and WhyCode fiducial systems in terms of orientation ambiguity and detection rate on embedded hardware. We test 2 April Tag variants - 1 default and 1 custom - and 3 Whycode variants - 1 default and 2 custom. We determine that they are suitable for autonomous drone landing applications in terms of detection rate, but may generate erroneous control signals as a result of orientation ambiguity in the pose estimates.

==> autogenerated/auto_generated_table_all.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Fiducial system & Test case & Detections & Discontinuities\\\hline
apriltag24h10 & in-out-1 & 942 & 73\\\hline
apriltag24h10 & in-out-2 & 671 & 55\\\hline
apriltag24h10 & east-west & 1209 & 25\\\hline
apriltag24h10 & calibration-z0.96 & 1937 & 42\\\hline
apriltag24h10 & north-south & 2001 & 61\\\hline
apriltag48h12 & calibration-z0.96 & 1938 & 0\\\hline
apriltag48h12 & north-south & 2005 & 0\\\hline
apriltag48h12 & in-out-2 & 668 & 0\\\hline
apriltag48h12 & in-out-1 & 948 & 2\\\hline
apriltag48h12 & east-west & 1207 & 0\\\hline
whycode-ellipse marker 0 & in-out-1 & 891 & 9\\\hline
whycode-ellipse marker 0 & north-south & 1846 & 9\\\hline
whycode-ellipse marker 0 & east-west & 1106 & 0\\\hline
whycode-ellipse marker 0 & calibration-z0.96 & 1798 & 0\\\hline
whycode-ellipse marker 0 & in-out-2 & 637 & 3\\\hline
whycode-ellipse marker 1 & in-out-1 & 891 & 27\\\hline
whycode-ellipse marker 1 & east-west & 1106 & 8\\\hline
whycode-ellipse marker 1 & in-out-2 & 637 & 0\\\hline
whycode-ellipse marker 1 & calibration-z0.96 & 1798 & 0\\\hline
whycode-ellipse marker 1 & north-south & 1846 & 2\\\hline
whycode-ellipse marker 2 & east-west & 1106 & 0\\\hline
whycode-ellipse marker 2 & in-out-1 & 891 & 13\\\hline
whycode-ellipse marker 2 & calibration-z0.96 & 1798 & 0\\\hline
whycode-ellipse marker 2 & in-out-2 & 637 & 17\\\hline
whycode-ellipse marker 2 & north-south & 1846 & 7\\\hline
whycode-multi & east-west & 1090 & 0\\\hline
whycode-multi & north-south & 1845 & 0\\\hline
whycode-multi & calibration-z0.96 & 1757 & 0\\\hline
whycode-multi & in-out-1 & 870 & 2\\\hline
whycode-multi & in-out-2 & 621 & 0\\\hline
whycode-orig marker 0 & north-south & 1852 & 53\\\hline
whycode-orig marker 0 & in-out-1 & 872 & 9\\\hline
whycode-orig marker 0 & east-west & 1127 & 129\\\hline
whycode-orig marker 0 & in-out-2 & 631 & 172\\\hline
whycode-orig marker 0 & calibration-z0.96 & 1773 & 820\\\hline
whycode-orig marker 1 & calibration-z0.96 & 1773 & 0\\\hline
whycode-orig marker 1 & in-out-2 & 631 & 55\\\hline
whycode-orig marker 1 & in-out-1 & 872 & 25\\\hline
whycode-orig marker 1 & north-south & 1852 & 2\\\hline
whycode-orig marker 1 & east-west & 1127 & 31\\\hline
whycode-orig marker 2 & in-out-2 & 631 & 130\\\hline
whycode-orig marker 2 & in-out-1 & 872 & 13\\\hline
whycode-orig marker 2 & calibration-z0.96 & 1773 & 0\\\hline
whycode-orig marker 2 & north-south & 1852 & 52\\\hline
whycode-orig marker 2 & east-west & 1127 & 92\\\hline
\end{tabular}
\caption{All aggregated data.}
\label{table:aggregated_data}
\end{table}


==> autogenerated/bundle_system_analysis_table.tex <==
\begin{tabular}{lrrrrrr}
\toprule
         Source &     SS &  DF &     MS &      F &  $p$ &    $\eta^2$ \\ \hline
\midrule
System & 0.0071 &   2 & 0.0035 & 11.249 & 0.0018 & 0.6522 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/bundle_system_data_table.tex <==
\begin{tabular}{llrrr}
\toprule
System &         Test Case &  $n$ &  $d$ &  $r_d$ \\ \hline
\midrule
  apriltag24h10 &          in-out-1 &         942 &               73 &            0.077495 \\ \hline
  apriltag24h10 &          in-out-2 &         671 &               55 &            0.081967 \\ \hline
  apriltag24h10 &         east-west &        1209 &               25 &            0.020678 \\ \hline
  apriltag24h10 & calibration-z0.96 &        1937 &               42 &            0.021683 \\ \hline
  apriltag24h10 &       north-south &        2001 &               61 &            0.030485 \\ \hline
  apriltag48h12 & calibration-z0.96 &        1938 &                0 &            0.000000 \\ \hline
  apriltag48h12 &       north-south &        2005 &                0 &            0.000000 \\ \hline
  apriltag48h12 &          in-out-2 &         668 &                0 &            0.000000 \\ \hline
  apriltag48h12 &          in-out-1 &         948 &                2 &            0.002110 \\ \hline
  apriltag48h12 &         east-west &        1207 &                0 &            0.000000 \\ \hline
  whycode-multi &         east-west &        1090 &                0 &            0.000000 \\ \hline
  whycode-multi &       north-south &        1845 &                0 &            0.000000 \\ \hline
  whycode-multi & calibration-z0.96 &        1757 &                0 &            0.000000 \\ \hline
  whycode-multi &          in-out-1 &         870 &                2 &            0.002299 \\ \hline
  whycode-multi &          in-out-2 &         621 &                0 &            0.000000 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/bundles_discontinuity_test_cases.tex <==
\begin{tabular}{|lrr|rrr|rrr|rrr|}
\toprule
         Test Case & Length (s) & Frames & \multicolumn{3}{c|}{April Tag 24h10} & \multicolumn{3}{c|}{April Tag 48h12} & \multicolumn{3}{c|}{WhyCode Multi} \\
                 &          &      &             $n$ & $d$ & $r_d$ &             $n$ & $d$ & $r_d$ &           $n$ & $d$ & $r_d$ \\
\midrule
 calibration-z1.42 &     30.769 &    924 &             924 &   0 & 0.000 &             924 &   0 & 0.000 &           807 &   0 & 0.000 \\
          in-out-1 &     20.862 &    627 &             627 &  89 & 0.142 &             627 &   0 & 0.000 &           552 &  20 & 0.036 \\
          in-out-2 &     17.630 &    530 &             530 & 154 & 0.291 &             530 &   1 & 0.002 &           465 &   0 & 0.000 \\
          in-out-3 &     20.697 &    622 &             622 & 181 & 0.291 &             622 &   2 & 0.003 &           542 &   1 & 0.002 \\
          in-out-4 &     24.062 &    723 &             723 & 341 & 0.472 &             723 &  54 & 0.075 &           641 & 146 & 0.228 \\
      left-right-1 &     28.330 &    851 &             851 &   6 & 0.007 &             851 &   0 & 0.000 &           748 &  30 & 0.040 \\
      left-right-2 &     24.865 &    747 &             747 &   2 & 0.003 &             747 &   0 & 0.000 &           652 &   1 & 0.002 \\
      left-right-3 &     22.731 &    683 &             683 &   0 & 0.000 &             683 &   0 & 0.000 &           597 &   0 & 0.000 \\
      left-right-4 &     20.499 &    616 &             616 & 290 & 0.471 &             616 &  51 & 0.083 &           553 & 138 & 0.250 \\
orbit-left-right-1 &     54.567 &   1638 &            1638 &  51 & 0.031 &            1638 &   0 & 0.000 &          1424 &   2 & 0.001 \\
orbit-left-right-2 &     41.096 &   1234 &            1234 & 107 & 0.087 &            1234 &   0 & 0.000 &          1074 &   2 & 0.002 \\
orbit-left-right-3 &     56.131 &   1685 &            1685 &  72 & 0.043 &            1685 &   0 & 0.000 &          1457 &   0 & 0.000 \\
orbit-left-right-4 &     40.833 &   1226 &            1226 & 350 & 0.285 &            1226 &  33 & 0.027 &          1079 & 109 & 0.101 \\
   orbit-up-down-1 &     91.032 &   2732 &            2732 &   3 & 0.001 &            2732 &   5 & 0.002 &          2396 &   0 & 0.000 \\
   orbit-up-down-2 &     80.296 &   2410 &            2410 &   5 & 0.002 &            2410 &   1 & 0.000 &          2089 &   0 & 0.000 \\
   orbit-up-down-3 &     55.998 &   1681 &            1681 &   0 & 0.000 &            1681 &   3 & 0.002 &          1469 &   0 & 0.000 \\
   orbit-up-down-4 &     58.999 &   1771 &            1771 & 374 & 0.211 &            1771 & 138 & 0.078 &          1557 & 300 & 0.193 \\
  pan-left-right-1 &     40.398 &   1213 &            1213 &  16 & 0.013 &            1213 &   2 & 0.002 &          1066 &  24 & 0.023 \\
  pan-left-right-2 &     43.829 &   1316 &            1316 &  27 & 0.021 &            1316 &  13 & 0.010 &          1156 &  19 & 0.016 \\
  pan-left-right-3 &     39.430 &   1184 &            1184 &  16 & 0.014 &            1184 &  10 & 0.008 &          1035 &  11 & 0.011 \\
  pan-left-right-4 &     28.563 &    858 &             858 & 322 & 0.375 &             858 &  86 & 0.100 &           759 & 254 & 0.335 \\
      randomized-1 &     39.730 &   1193 &            1193 & 401 & 0.336 &            1193 &  39 & 0.033 &           991 &   5 & 0.005 \\
      randomized-2 &     24.365 &    732 &             732 & 257 & 0.351 &             732 &  16 & 0.022 &           582 &  43 & 0.074 \\
      randomized-3 &     31.199 &    937 &             937 & 381 & 0.407 &             937 &  52 & 0.055 &           718 &  44 & 0.061 \\
      randomized-4 &     36.799 &   1105 &            1105 & 460 & 0.416 &            1105 & 168 & 0.152 &           814 & 162 & 0.199 \\
    tilt-up-down-1 &     29.998 &    901 &             901 &   0 & 0.000 &             901 &   0 & 0.000 &           793 &   0 & 0.000 \\
    tilt-up-down-2 &     41.301 &   1240 &            1240 &  53 & 0.043 &            1240 &  16 & 0.013 &          1083 &  11 & 0.010 \\
    tilt-up-down-3 &     29.632 &    890 &             890 &  40 & 0.045 &             890 &  21 & 0.024 &           779 &   0 & 0.000 \\
    tilt-up-down-4 &     37.931 &   1139 &            1139 & 367 & 0.322 &            1139 & 100 & 0.088 &          1000 & 267 & 0.267 \\
         up-down-1 &     33.167 &    996 &             996 &  50 & 0.050 &             996 &   3 & 0.003 &           874 &   0 & 0.000 \\
         up-down-2 &     31.998 &    961 &             961 & 223 & 0.232 &             961 &  10 & 0.010 &           845 &   0 & 0.000 \\
         up-down-3 &     39.030 &   1172 &            1172 & 132 & 0.113 &            1172 &   1 & 0.001 &          1039 &   0 & 0.000 \\
         up-down-4 &     33.298 &   1000 &            1000 & 247 & 0.247 &            1000 &  72 & 0.072 &           883 & 233 & 0.264 \\
\bottomrule
\end{tabular}


==> autogenerated/bundles_speed_test_cases.tex <==
\begin{tabular}{|l|rrr|rrr|rrr|rrr|}
\toprule
Fiducial System & \multicolumn{3}{c|}{April Tag 24h10} & \multicolumn{3}{c|}{April Tag 48h12} & \multicolumn{3}{c|}{WhyCode Multi} \\
{} &      $\ell$ (s) &  $n$ & $F$ (Hz) &      $\ell$ (s) &  $n$ & $F$ (Hz) &    $\ell$ (s) &  $n$ & $F$ (Hz) \\
Test Case           &                 &      &          &                 &      &          &               &      &          \\
\midrule
z120cm-0            &            19.9 &  340 &     17.1 &            19.9 &  315 &     15.9 &          19.9 &  504 &     25.3 \\
z120cm-1            &            19.9 &  354 &     17.8 &            19.9 &  316 &     15.9 &          19.9 &  515 &     25.9 \\
z120cm-2            &            19.9 &  349 &     17.6 &            19.9 &  313 &     15.8 &          19.9 &  508 &     25.5 \\
z120cm-deflection-0 &            19.9 &  354 &     17.8 &            19.9 &  395 &     19.9 &          19.9 &  502 &     25.2 \\
z120cm-deflection-1 &            19.9 &  365 &     18.4 &            19.9 &  391 &     19.7 &          19.9 &  513 &     25.8 \\
z120cm-deflection-2 &            19.9 &  319 &     16.1 &            19.9 &  390 &     19.6 &          19.9 &  510 &     25.6 \\
z150cm-0            &            19.8 &  354 &     17.8 &            19.8 &  296 &     15.0 &          19.9 &  387 &     19.5 \\
z150cm-1            &            19.8 &  376 &     18.9 &            19.8 &  358 &     18.1 &          19.9 &  353 &     17.8 \\
z150cm-2            &            19.8 &  367 &     18.5 &            19.8 &  362 &     18.3 &          19.9 &  386 &     19.4 \\
z150cm-deflection-0 &            19.9 &  379 &     19.1 &            19.9 &  345 &     17.4 &          19.9 &  393 &     19.7 \\
z150cm-deflection-1 &            19.9 &  374 &     18.8 &            19.9 &  355 &     17.9 &          19.9 &  392 &     19.7 \\
z150cm-deflection-2 &            19.9 &  378 &     19.0 &            19.9 &  364 &     18.3 &          19.9 &  388 &     19.5 \\
z180cm-0            &            19.9 &  305 &     15.4 &            19.9 &  327 &     16.5 &          19.9 &  518 &     26.0 \\
z180cm-1            &            19.9 &  300 &     15.1 &            19.9 &  324 &     16.3 &          19.9 &  513 &     25.8 \\
z180cm-2            &            19.9 &  308 &     15.5 &            19.9 &  325 &     16.4 &          19.9 &  518 &     26.0 \\
z180cm-deflection-0 &            19.9 &  342 &     17.2 &            19.8 &  348 &     17.5 &          19.9 &  517 &     26.0 \\
z180cm-deflection-1 &            19.9 &  328 &     16.5 &            19.8 &  355 &     17.9 &          19.9 &  515 &     25.9 \\
z180cm-deflection-2 &            19.9 &  370 &     18.6 &            19.8 &  359 &     18.1 &          19.9 &  514 &     25.8 \\
z210cm-0            &            19.9 &  352 &     17.7 &            19.9 &  337 &     17.0 &          19.9 &  398 &     20.0 \\
z210cm-1            &            19.9 &  350 &     17.6 &            19.9 &  344 &     17.3 &          19.9 &  395 &     19.9 \\
z210cm-2            &            19.9 &  340 &     17.1 &            19.9 &  338 &     17.0 &          19.9 &  394 &     19.8 \\
z210cm-deflection-0 &            19.9 &  324 &     16.3 &            19.9 &  316 &     15.9 &          19.9 &  388 &     19.5 \\
z210cm-deflection-1 &            19.9 &  331 &     16.7 &            19.9 &  313 &     15.8 &          19.9 &  395 &     19.9 \\
z210cm-deflection-2 &            19.9 &  335 &     16.9 &            19.9 &  335 &     16.9 &          19.9 &  390 &     19.6 \\
z240cm-0            &            19.9 &  283 &     14.2 &            19.8 &  293 &     14.8 &          19.9 &  503 &     25.3 \\
z240cm-1            &            19.9 &  296 &     14.9 &            19.8 &  295 &     14.9 &          19.9 &  519 &     26.1 \\
z240cm-2            &            19.9 &  256 &     12.9 &            19.8 &  296 &     14.9 &          19.9 &  519 &     26.1 \\
z240cm-deflection-0 &            19.9 &  258 &     13.0 &            19.9 &  299 &     15.1 &          19.9 &  519 &     26.1 \\
z240cm-deflection-1 &            19.9 &  298 &     15.0 &            19.9 &  299 &     15.1 &          19.9 &  517 &     26.0 \\
z240cm-deflection-2 &            19.9 &  300 &     15.1 &            19.9 &  301 &     15.2 &          19.9 &  513 &     25.8 \\
z270cm-0            &            19.9 &  304 &     15.3 &            19.9 &  291 &     14.6 &          19.9 &  383 &     19.3 \\
z270cm-1            &            19.9 &  303 &     15.3 &            19.9 &  295 &     14.8 &          19.9 &  303 &     15.2 \\
z270cm-2            &            19.9 &  303 &     15.3 &            19.9 &  297 &     15.0 &          19.9 &  391 &     19.7 \\
z270cm-deflection-0 &            19.9 &  297 &     15.0 &            19.9 &  285 &     14.3 &          19.9 &  369 &     18.5 \\
z270cm-deflection-1 &            19.9 &  281 &     14.1 &            19.9 &  296 &     14.9 &          19.9 &  329 &     16.5 \\
z270cm-deflection-2 &            19.9 &  299 &     15.1 &            19.9 &  298 &     15.0 &          19.9 &  367 &     18.4 \\
z300cm-0            &            19.9 &  285 &     14.3 &            19.9 &  298 &     15.0 &          19.9 &  477 &     24.0 \\
z300cm-1            &            19.9 &  278 &     14.0 &            19.9 &  298 &     15.0 &          19.9 &  516 &     25.9 \\
z300cm-2            &            19.9 &  289 &     14.5 &            19.9 &  297 &     14.9 &          19.9 &  520 &     26.1 \\
z300cm-deflection-0 &            19.9 &  294 &     14.8 &            19.9 &  294 &     14.8 &          19.9 &  508 &     25.5 \\
z300cm-deflection-1 &            19.9 &  286 &     14.4 &            19.9 &  294 &     14.8 &          19.9 &  519 &     26.1 \\
z300cm-deflection-2 &            19.9 &  247 &     12.4 &            19.9 &  293 &     14.8 &          19.9 &  518 &     26.0 \\
\bottomrule
\end{tabular}


==> autogenerated/individual_system_analysis_table.tex <==
\begin{tabular}{lrrrrrr}
\toprule
         Source &     SS &  DF &     MS &      F &  $p$ &    $\eta^2$ \\ \hline
\midrule
System & 0.0176 &   1 & 0.0176 & 5.7639 & 0.0431 & 0.4188 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/individual_system_data_table.tex <==
\begin{tabular}{llrrr}
\toprule
System &         Test Case &  $n$ &  $d$ &  $r_d$ \\ \hline
\midrule
whycode-ellipse & calibration-z0.96 &        5394 &                0 &            0.000000 \\ \hline
whycode-ellipse &         east-west &        3318 &                8 &            0.002411 \\ \hline
whycode-ellipse &          in-out-1 &        2673 &               49 &            0.018331 \\ \hline
whycode-ellipse &          in-out-2 &        1911 &               20 &            0.010466 \\ \hline
whycode-ellipse &       north-south &        5538 &               18 &            0.003250 \\ \hline
   whycode-orig & calibration-z0.96 &        5319 &              820 &            0.154164 \\ \hline
   whycode-orig &         east-west &        3381 &              252 &            0.074534 \\ \hline
   whycode-orig &          in-out-1 &        2616 &               47 &            0.017966 \\ \hline
   whycode-orig &          in-out-2 &        1893 &              357 &            0.188590 \\ \hline
   whycode-orig &       north-south &        5556 &              107 &            0.019258 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/kruskal_bundles.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &      $H$ \\
\midrule
       0.000675 & 14.60195 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_five_member.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &       $H$ \\
\midrule
       0.000033 & 25.935888 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_intra_whycode.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &       $H$ \\
\midrule
       0.000321 & 16.088998 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_single_marker.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &       $H$ \\
\midrule
       0.000025 & 23.980363 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_speed_bundles.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &       $H$ \\
\midrule
   5.212361e-16 & 70.380657 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_speed_five_member.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &       $H$ \\
\midrule
   2.275795e-11 & 55.737741 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_speed_single_marker.tex <==
\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &        $H$ \\
\midrule
   2.982518e-27 & 126.558803 \\
\bottomrule
\end{tabular}


==> autogenerated/kruskal_wallis.tex <==
\todo[inline]{switch headers obviously \\}

\begin{tabular}{rr}
\toprule
 $p_{\forall=}$ &     $H$ \\ \hline
\midrule
      18.099205 & 0.00118 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/mann_whitney_pairwise.tex <==
\begin{tabular}{llrrr}
\toprule
System 1 & System 2 &  $U_1$ &  $U_2$ &  $p$ \\ \hline
\midrule
   apriltag24h10 &    apriltag48h12 &         25.0 &          0.0 &    0.011 \\ \hline
   apriltag24h10 &  whycode-ellipse &         25.0 &          0.0 &    0.008 \\ \hline
   apriltag24h10 &    whycode-multi &         25.0 &          0.0 &    0.010 \\ \hline
   apriltag24h10 &     whycode-orig &         13.0 &         12.0 &    1.000 \\ \hline
   apriltag48h12 &    apriltag24h10 &          0.0 &         25.0 &    0.011 \\ \hline
   apriltag48h12 &  whycode-ellipse &         11.5 &         13.5 &    0.914 \\ \hline
   apriltag48h12 &    whycode-multi &         16.0 &          9.0 &    0.441 \\ \hline
   apriltag48h12 &     whycode-orig &          2.0 &         23.0 &    0.034 \\ \hline
 whycode-ellipse &    apriltag24h10 &          0.0 &         25.0 &    0.008 \\ \hline
 whycode-ellipse &    apriltag48h12 &         13.5 &         11.5 &    0.914 \\ \hline
 whycode-ellipse &    whycode-multi &         22.0 &          3.0 &    0.045 \\ \hline
 whycode-ellipse &     whycode-orig &          0.0 &         25.0 &    0.008 \\ \hline
   whycode-multi &    apriltag24h10 &          0.0 &         25.0 &    0.010 \\ \hline
   whycode-multi &    apriltag48h12 &          9.0 &         16.0 &    0.441 \\ \hline
   whycode-multi &  whycode-ellipse &          3.0 &         22.0 &    0.045 \\ \hline
   whycode-multi &     whycode-orig &          0.0 &         25.0 &    0.010 \\ \hline
    whycode-orig &    apriltag24h10 &         12.0 &         13.0 &    1.000 \\ \hline
    whycode-orig &    apriltag48h12 &         23.0 &          2.0 &    0.034 \\ \hline
    whycode-orig &  whycode-ellipse &         25.0 &          0.0 &    0.008 \\ \hline
    whycode-orig &    whycode-multi &         25.0 &          0.0 &    0.010 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/mann_wilcox_pairwise.tex <==
\begin{tabular}{llrrr}
\toprule
System 1 & System 2 &  $U_1$ &  $U_2$ &  $p$ \\ \hline
\midrule
   apriltag24h10 &    apriltag48h12 &         25.0 &          0.0 &    0.011 \\ \hline
   apriltag24h10 &  whycode-ellipse &         25.0 &          0.0 &    0.008 \\ \hline
   apriltag24h10 &    whycode-multi &         25.0 &          0.0 &    0.010 \\ \hline
   apriltag24h10 &     whycode-orig &         13.0 &         12.0 &    1.000 \\ \hline
   apriltag48h12 &    apriltag24h10 &          0.0 &         25.0 &    0.011 \\ \hline
   apriltag48h12 &  whycode-ellipse &         11.5 &         13.5 &    0.914 \\ \hline
   apriltag48h12 &    whycode-multi &         16.0 &          9.0 &    0.441 \\ \hline
   apriltag48h12 &     whycode-orig &          2.0 &         23.0 &    0.034 \\ \hline
 whycode-ellipse &    apriltag24h10 &          0.0 &         25.0 &    0.008 \\ \hline
 whycode-ellipse &    apriltag48h12 &         13.5 &         11.5 &    0.914 \\ \hline
 whycode-ellipse &    whycode-multi &         22.0 &          3.0 &    0.045 \\ \hline
 whycode-ellipse &     whycode-orig &          0.0 &         25.0 &    0.008 \\ \hline
   whycode-multi &    apriltag24h10 &          0.0 &         25.0 &    0.010 \\ \hline
   whycode-multi &    apriltag48h12 &          9.0 &         16.0 &    0.441 \\ \hline
   whycode-multi &  whycode-ellipse &          3.0 &         22.0 &    0.045 \\ \hline
   whycode-multi &     whycode-orig &          0.0 &         25.0 &    0.010 \\ \hline
    whycode-orig &    apriltag24h10 &         12.0 &         13.0 &    1.000 \\ \hline
    whycode-orig &    apriltag48h12 &         23.0 &          2.0 &    0.034 \\ \hline
    whycode-orig &  whycode-ellipse &         25.0 &          0.0 &    0.008 \\ \hline
    whycode-orig &    whycode-multi &         25.0 &          0.0 &    0.010 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/orig.bundle_system_analysis_table.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    sum\_sq &   df &         F &    PR(>F) \\ \hline
\midrule
C(fiducial\_system) &  0.007060 &  2.0 &  11.68560 &  0.004229 \\ \hline
C(test\_case)       &  0.001349 &  4.0 &   1.11644 &  0.412688 \\ \hline
Residual           &  0.002417 &  8.0 &       NaN &       NaN \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/orig.bundle_system_data_table.tex <==
\begin{tabular}{llrrr}
\toprule
       System &         Test Case &    $n$ &  $d$ &      $r_d$ \\ \hline
\midrule
apriltag24h10 &          in-out-1 &  942 &   73 & 0.077495 \\ \hline
apriltag24h10 &          in-out-2 &  671 &   55 & 0.081967 \\ \hline
apriltag24h10 &         east-west & 1209 &   25 & 0.020678 \\ \hline
apriltag24h10 & calibration-z0.96 & 1937 &   42 & 0.021683 \\ \hline
apriltag24h10 &       north-south & 2001 &   61 & 0.030485 \\ \hline
apriltag48h12 & calibration-z0.96 & 1938 &    0 & 0.000000 \\ \hline
apriltag48h12 &       north-south & 2005 &    0 & 0.000000 \\ \hline
apriltag48h12 &          in-out-2 &  668 &    0 & 0.000000 \\ \hline
apriltag48h12 &          in-out-1 &  948 &    2 & 0.002110 \\ \hline
apriltag48h12 &         east-west & 1207 &    0 & 0.000000 \\ \hline
whycode-multi &         east-west & 1090 &    0 & 0.000000 \\ \hline
whycode-multi &       north-south & 1845 &    0 & 0.000000 \\ \hline
whycode-multi & calibration-z0.96 & 1757 &    0 & 0.000000 \\ \hline
whycode-multi &          in-out-1 &  870 &    2 & 0.002299 \\ \hline
whycode-multi &          in-out-2 &  621 &    0 & 0.000000 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/orig.individual_system_analysis_table.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    sum\_sq &   df &        F &    PR(>F) \\ \hline
\midrule
C(fiducial\_system) &  0.017645 &  1.0 &  5.50023 &  0.078923 \\ \hline
C(test\_case)       &  0.011658 &  4.0 &  0.90851 &  0.535926 \\ \hline
Residual           &  0.012832 &  4.0 &      NaN &       NaN \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/orig.individual_system_data_table.tex <==
\begin{tabular}{llrrr}
\toprule
fiducial\_system &         test\_case &  $n$ &  $d$ &  $r_d$ \\ \hline
\midrule
whycode-ellipse & calibration-z0.96 &        5394 &                0 &            0.000000 \\ \hline
whycode-ellipse &         east-west &        3318 &                8 &            0.002411 \\ \hline
whycode-ellipse &          in-out-1 &        2673 &               49 &            0.018331 \\ \hline
whycode-ellipse &          in-out-2 &        1911 &               20 &            0.010466 \\ \hline
whycode-ellipse &       north-south &        5538 &               18 &            0.003250 \\ \hline
   whycode-orig & calibration-z0.96 &        5319 &              820 &            0.154164 \\ \hline
   whycode-orig &         east-west &        3381 &              252 &            0.074534 \\ \hline
   whycode-orig &          in-out-1 &        2616 &               47 &            0.017966 \\ \hline
   whycode-orig &          in-out-2 &        1893 &              357 &            0.188590 \\ \hline
   whycode-orig &       north-south &        5556 &              107 &            0.019258 \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/single_marker_discontinuity_test_cases.tex <==
\begin{tabular}{|lrr|rrr|rrr|rrr|rrr|}
\toprule
         Test Case & Length (s) & Frames & \multicolumn{3}{c|}{April Tag 24h10} & \multicolumn{3}{c|}{April Tag 48h12} & \multicolumn{3}{c|}{WhyCode Ellipse} & \multicolumn{3}{c|}{WhyCode Orig} \\
                 &          &      &             $n$ & $d$ & $r_d$ &             $n$ & $d$ & $r_d$ &             $n$ & $d$ & $r_d$ &          $n$ & $d$ & $r_d$ \\
\midrule
 calibration-z1.42 &     30.769 &    924 &             924 &   0 & 0.000 &             924 &   0 & 0.000 &             922 &   0 & 0.000 &          918 &   0 & 0.000 \\
          in-out-1 &     20.862 &    627 &             627 &  91 & 0.145 &             627 &   0 & 0.000 &             624 &   1 & 0.002 &          627 &   1 & 0.002 \\
          in-out-2 &     17.630 &    530 &             530 & 161 & 0.304 &             530 &   1 & 0.002 &             524 &   0 & 0.000 &          530 &   0 & 0.000 \\
          in-out-3 &     20.697 &    622 &             622 & 167 & 0.268 &             622 &   2 & 0.003 &             620 &   0 & 0.000 &          620 &   0 & 0.000 \\
          in-out-4 &     24.062 &    723 &             723 & 340 & 0.470 &             723 &  54 & 0.075 &             721 &   0 & 0.000 &          719 &  63 & 0.088 \\
      left-right-1 &     28.330 &    851 &             851 &   7 & 0.008 &             851 &   0 & 0.000 &             848 &  12 & 0.014 &          850 & 148 & 0.174 \\
      left-right-2 &     24.865 &    747 &             747 &   1 & 0.001 &             747 &   1 & 0.001 &             746 &   0 & 0.000 &          744 &   0 & 0.000 \\
      left-right-3 &     22.731 &    683 &             683 &   0 & 0.000 &             683 &   0 & 0.000 &             681 &   0 & 0.000 &          679 &   0 & 0.000 \\
      left-right-4 &     20.499 &    616 &             616 & 290 & 0.471 &             616 &  51 & 0.083 &             615 &   3 & 0.005 &          615 &  72 & 0.117 \\
orbit-left-right-1 &     54.567 &   1638 &            1638 &  34 & 0.021 &            1638 &   0 & 0.000 &            1631 &   0 & 0.000 &         1635 &   0 & 0.000 \\
orbit-left-right-2 &     41.096 &   1234 &            1234 &   0 & 0.000 &            1234 &   0 & 0.000 &            1229 &   0 & 0.000 &         1229 &   0 & 0.000 \\
orbit-left-right-3 &     56.131 &   1685 &            1685 &  73 & 0.043 &            1685 &   0 & 0.000 &            1681 &   0 & 0.000 &         1682 &   0 & 0.000 \\
orbit-left-right-4 &     40.833 &   1226 &            1226 & 350 & 0.285 &            1226 &  33 & 0.027 &            1220 &  16 & 0.013 &         1225 &  84 & 0.069 \\
   orbit-up-down-1 &     91.032 &   2732 &            2732 &   7 & 0.003 &            2732 &   0 & 0.000 &            2709 &   0 & 0.000 &         2724 &   0 & 0.000 \\
   orbit-up-down-2 &     80.296 &   2410 &            2410 &   6 & 0.002 &            2410 &   2 & 0.001 &            2403 &   0 & 0.000 &         2402 &   0 & 0.000 \\
   orbit-up-down-3 &     55.998 &   1681 &            1681 &   0 & 0.000 &            1681 &   0 & 0.000 &            1645 &   0 & 0.000 &         1671 &   0 & 0.000 \\
   orbit-up-down-4 &     58.999 &   1771 &            1771 & 374 & 0.211 &            1771 & 135 & 0.076 &            1761 &  48 & 0.027 &         1760 & 188 & 0.107 \\
  pan-left-right-1 &     40.398 &   1213 &            1213 &  18 & 0.015 &            1213 &   4 & 0.003 &            1205 &   4 & 0.003 &         1207 & 109 & 0.090 \\
  pan-left-right-2 &     43.829 &   1316 &            1316 &  28 & 0.021 &            1316 &  18 & 0.014 &            1308 &   0 & 0.000 &         1311 &  79 & 0.060 \\
  pan-left-right-3 &     39.430 &   1184 &            1184 &  18 & 0.015 &            1184 &   8 & 0.007 &            1179 &   2 & 0.002 &         1183 &  64 & 0.054 \\
  pan-left-right-4 &     28.563 &    858 &             858 & 322 & 0.375 &             858 &  86 & 0.100 &             858 &  76 & 0.089 &          858 & 174 & 0.203 \\
      randomized-1 &     39.730 &   1193 &            1193 & 377 & 0.316 &            1193 &  30 & 0.025 &            1183 &   1 & 0.001 &         1186 &   0 & 0.000 \\
      randomized-2 &     24.365 &    732 &             732 & 257 & 0.351 &             732 &  16 & 0.022 &             725 &  20 & 0.028 &          726 &  24 & 0.033 \\
      randomized-3 &     31.199 &    937 &             937 & 382 & 0.408 &             937 &  51 & 0.054 &             930 &  50 & 0.054 &          929 &  73 & 0.079 \\
      randomized-4 &     36.799 &   1105 &            1105 & 460 & 0.416 &            1105 & 168 & 0.152 &            1094 & 109 & 0.100 &         1093 & 129 & 0.118 \\
    tilt-up-down-1 &     29.998 &    901 &             901 &   8 & 0.009 &             901 &   0 & 0.000 &             897 &   0 & 0.000 &          897 &   0 & 0.000 \\
    tilt-up-down-2 &     41.301 &   1240 &            1240 &  57 & 0.046 &            1240 &   0 & 0.000 &            1234 &   1 & 0.001 &         1237 &  93 & 0.075 \\
    tilt-up-down-3 &     29.632 &    890 &             890 &  53 & 0.060 &             890 &   4 & 0.004 &             886 &   0 & 0.000 &          886 &   0 & 0.000 \\
    tilt-up-down-4 &     37.931 &   1139 &            1139 & 367 & 0.322 &            1139 & 100 & 0.088 &            1134 &  81 & 0.071 &         1137 & 355 & 0.312 \\
         up-down-1 &     33.167 &    996 &             996 &  70 & 0.070 &             996 &  10 & 0.010 &             993 &   0 & 0.000 &          993 &   0 & 0.000 \\
         up-down-2 &     31.998 &    961 &             961 & 216 & 0.225 &             961 &  21 & 0.022 &             958 &   0 & 0.000 &          958 &   0 & 0.000 \\
         up-down-3 &     39.030 &   1172 &            1172 &  87 & 0.074 &            1172 &   0 & 0.000 &            1166 &   0 & 0.000 &         1168 &   0 & 0.000 \\
         up-down-4 &     33.298 &   1000 &            1000 & 247 & 0.247 &            1000 &  70 & 0.070 &             999 &  58 & 0.058 &          999 & 279 & 0.279 \\
\bottomrule
\end{tabular}


==> autogenerated/single_marker_speed_test_cases.tex <==
\begin{tabular}{|l|rrr|rrr|rrr|rrr|}
\toprule
Fiducial System & \multicolumn{3}{c|}{April Tag 24h10} & \multicolumn{3}{c|}{April Tag 48h12} & \multicolumn{3}{c|}{WhyCode Ellipse} & \multicolumn{3}{c|}{WhyCode Orig} \\
{} &      $\ell$ (s) &  $n$ & $F$ (Hz) &      $\ell$ (s) &  $n$ & $F$ (Hz) &      $\ell$ (s) &  $n$ & $F$ (Hz) &   $\ell$ (s) &  $n$ & $F$ (Hz) \\
Test Case           &                 &      &          &                 &      &          &                 &      &          &              &      &          \\
\midrule
z120cm-0            &            19.9 &  374 &     18.8 &            19.9 &  340 &     17.1 &            19.9 &  509 &     25.6 &         19.9 &  512 &     25.7 \\
z120cm-1            &            19.9 &  379 &     19.1 &            19.9 &  328 &     16.5 &            19.9 &  509 &     25.6 &         19.9 &  516 &     25.9 \\
z120cm-2            &            19.9 &  384 &     19.3 &            19.9 &  336 &     16.9 &            19.9 &  513 &     25.8 &         19.9 &  518 &     26.0 \\
z120cm-deflection-0 &            19.9 &  397 &     20.0 &            19.9 &  356 &     17.9 &            19.9 &  515 &     25.9 &         19.9 &  519 &     26.1 \\
z120cm-deflection-1 &            19.9 &  417 &     21.0 &            19.9 &  398 &     20.0 &            19.9 &  518 &     26.0 &         19.9 &  521 &     26.2 \\
z120cm-deflection-2 &            19.9 &  410 &     20.6 &            19.9 &  412 &     20.7 &            19.9 &  514 &     25.8 &         19.9 &  521 &     26.2 \\
z150cm-0            &            19.9 &  380 &     19.1 &            19.9 &  429 &     21.6 &            19.9 &  514 &     25.8 &         19.9 &  529 &     26.6 \\
z150cm-1            &            19.9 &  370 &     18.6 &            19.9 &  422 &     21.2 &            19.9 &  520 &     26.1 &         19.9 &  518 &     26.0 \\
z150cm-2            &            19.9 &  357 &     18.0 &            19.9 &  425 &     21.4 &            19.9 &  519 &     26.1 &         19.9 &  522 &     26.2 \\
z150cm-deflection-0 &            19.9 &  368 &     18.5 &            19.9 &  420 &     21.1 &            19.9 &  512 &     25.7 &         19.9 &  518 &     26.1 \\
z150cm-deflection-1 &            19.9 &  370 &     18.6 &            19.9 &  429 &     21.6 &            19.9 &  522 &     26.3 &         19.9 &  525 &     26.4 \\
z150cm-deflection-2 &            19.9 &  379 &     19.0 &            19.9 &  429 &     21.6 &            19.9 &  516 &     25.9 &         19.9 &  527 &     26.5 \\
z180cm-0            &            19.9 &  348 &     17.5 &            19.9 &  330 &     16.6 &            19.9 &  521 &     26.2 &         19.9 &  527 &     26.5 \\
z180cm-1            &            19.9 &  336 &     16.9 &            19.9 &  329 &     16.6 &            19.9 &  521 &     26.2 &         19.9 &  528 &     26.5 \\
z180cm-2            &            19.9 &  346 &     17.4 &            19.9 &  335 &     16.9 &            19.9 &  526 &     26.4 &         19.9 &  523 &     26.3 \\
z180cm-deflection-0 &            19.9 &  385 &     19.4 &            19.8 &  354 &     17.8 &            19.9 &  516 &     25.9 &         19.9 &  516 &     25.9 \\
z180cm-deflection-1 &            19.9 &  377 &     19.0 &            19.8 &  345 &     17.4 &            19.9 &  514 &     25.8 &         19.9 &  512 &     25.7 \\
z180cm-deflection-2 &            19.9 &  393 &     19.8 &            19.8 &  362 &     18.3 &            19.9 &  522 &     26.2 &         19.9 &  522 &     26.2 \\
z210cm-0            &            19.9 &  342 &     17.2 &            19.9 &  409 &     20.6 &            19.9 &  519 &     26.1 &         19.9 &  485 &     24.4 \\
z210cm-1            &            19.9 &  345 &     17.4 &            19.9 &  398 &     20.0 &            19.9 &  524 &     26.3 &         19.9 &  503 &     25.3 \\
z210cm-2            &            19.9 &  340 &     17.1 &            19.9 &  397 &     20.0 &            19.9 &  518 &     26.0 &         19.9 &  522 &     26.2 \\
z210cm-deflection-0 &            19.9 &  321 &     16.2 &            19.9 &  378 &     19.0 &            19.9 &  522 &     26.2 &         19.9 &  456 &     22.9 \\
z210cm-deflection-1 &            19.9 &  330 &     16.6 &            19.9 &  380 &     19.1 &            19.9 &  521 &     26.2 &         19.9 &  527 &     26.5 \\
z210cm-deflection-2 &            19.9 &  326 &     16.4 &            19.9 &  379 &     19.1 &            19.9 &  523 &     26.3 &         19.9 &  525 &     26.4 \\
z240cm-0            &            19.9 &  288 &     14.5 &            19.9 &  293 &     14.8 &            19.9 &  531 &     26.7 &         19.9 &  526 &     26.4 \\
z240cm-1            &            19.9 &  299 &     15.0 &            19.9 &  295 &     14.9 &            19.9 &  522 &     26.2 &         19.9 &  534 &     26.8 \\
z240cm-2            &            19.9 &  298 &     15.0 &            19.9 &  298 &     15.0 &            19.9 &  522 &     26.2 &         19.9 &  524 &     26.3 \\
z240cm-deflection-0 &            19.9 &  313 &     15.7 &            19.9 &  295 &     14.8 &            19.9 &  526 &     26.4 &         19.9 &  531 &     26.7 \\
z240cm-deflection-1 &            19.9 &  316 &     15.9 &            19.9 &  299 &     15.0 &            19.9 &  524 &     26.3 &         19.9 &  525 &     26.4 \\
z240cm-deflection-2 &            19.9 &  315 &     15.8 &            19.9 &  298 &     15.0 &            19.9 &  524 &     26.3 &         19.9 &  526 &     26.4 \\
z270cm-0            &            19.9 &  297 &     14.9 &            19.9 &  328 &     16.5 &            19.9 &  520 &     26.1 &         19.9 &  519 &     26.1 \\
z270cm-1            &            19.9 &  298 &     15.0 &            19.9 &  317 &     15.9 &            19.9 &  523 &     26.3 &         19.9 &  524 &     26.3 \\
z270cm-2            &            19.9 &  297 &     14.9 &            19.9 &  319 &     16.0 &            19.9 &  518 &     26.0 &         19.9 &  543 &     27.3 \\
z270cm-deflection-0 &            19.9 &  295 &     14.9 &            19.9 &  310 &     15.6 &            19.9 &  445 &     22.4 &         19.9 &  532 &     26.7 \\
z270cm-deflection-1 &            19.9 &  298 &     15.0 &            19.9 &  313 &     15.7 &            19.9 &  529 &     26.6 &         19.9 &  529 &     26.6 \\
z270cm-deflection-2 &            19.9 &  294 &     14.8 &            19.9 &  312 &     15.7 &            19.9 &  520 &     26.1 &         19.9 &  522 &     26.2 \\
z300cm-0            &            19.9 &  299 &     15.0 &            19.9 &  289 &     14.5 &            19.9 &  526 &     26.4 &         19.9 &  521 &     26.2 \\
z300cm-1            &            19.9 &  299 &     15.0 &            19.9 &  296 &     14.9 &            19.9 &  523 &     26.3 &         19.9 &  526 &     26.4 \\
z300cm-2            &            19.9 &  299 &     15.0 &            19.9 &  298 &     15.0 &            19.9 &  523 &     26.3 &         19.9 &  529 &     26.6 \\
z300cm-deflection-0 &            19.9 &  299 &     15.0 &            19.9 &  290 &     14.6 &            19.9 &  528 &     26.5 &         19.9 &  537 &     27.0 \\
z300cm-deflection-1 &            19.9 &  295 &     14.8 &            19.9 &  294 &     14.8 &            19.9 &  523 &     26.2 &         19.9 &  526 &     26.4 \\
z300cm-deflection-2 &            19.9 &  299 &     15.0 &            19.9 &  294 &     14.8 &            19.9 &  530 &     26.6 &         19.9 &  528 &     26.5 \\
\bottomrule
\end{tabular}


==> autogenerated/speed_test_cases.tex <==
\begin{tabular}{lrll}
\toprule
        test\_case &  length\_sec & frames & fiducial\_system \\
\midrule
           z060cm &        59.7 &   1793 &   apriltag24h10 \\
z060cm-deflection &        59.7 &   1793 &   apriltag24h10 \\
           z120cm &        59.7 &   1792 &   apriltag24h10 \\
z120cm-deflection &        59.7 &   1792 &   apriltag24h10 \\
           z150cm &        59.8 &   1794 &   apriltag24h10 \\
z150cm-deflection &        59.7 &   1792 &   apriltag24h10 \\
           z180cm &        59.7 &   1793 &   apriltag24h10 \\
z180cm-deflection &        59.7 &   1792 &   apriltag24h10 \\
           z210cm &        59.7 &   1792 &   apriltag24h10 \\
z210cm-deflection &        59.7 &   1792 &   apriltag24h10 \\
           z240cm &        59.7 &   1791 &   apriltag24h10 \\
z240cm-deflection &        59.7 &   1793 &   apriltag24h10 \\
           z270cm &        59.7 &   1792 &   apriltag24h10 \\
z270cm-deflection &        59.7 &   1792 &   apriltag24h10 \\
           z300cm &        59.7 &   1792 &   apriltag24h10 \\
z300cm-deflection &        59.7 &   1792 &   apriltag24h10 \\
           z060cm &        59.7 &   1791 &   apriltag48h12 \\
z060cm-deflection &        59.7 &   1791 &   apriltag48h12 \\
           z120cm &        59.7 &   1792 &   apriltag48h12 \\
z120cm-deflection &        59.7 &   1793 &   apriltag48h12 \\
           z150cm &        59.7 &   1791 &   apriltag48h12 \\
z150cm-deflection &        59.7 &   1793 &   apriltag48h12 \\
           z180cm &        59.7 &   1792 &   apriltag48h12 \\
z180cm-deflection &        59.7 &   1791 &   apriltag48h12 \\
           z210cm &        59.7 &   1792 &   apriltag48h12 \\
z210cm-deflection &        59.8 &   1794 &   apriltag48h12 \\
           z240cm &        59.8 &   1793 &   apriltag48h12 \\
z240cm-deflection &        59.7 &   1792 &   apriltag48h12 \\
           z270cm &        59.7 &   1792 &   apriltag48h12 \\
z270cm-deflection &        59.8 &   1794 &   apriltag48h12 \\
           z300cm &        59.8 &   1794 &   apriltag48h12 \\
z300cm-deflection &        59.7 &   1792 &   apriltag48h12 \\
           z060cm &        59.7 &   1792 &   whycode-multi \\
z060cm-deflection &        59.8 &   1794 &   whycode-multi \\
           z120cm &        59.7 &   1793 &   whycode-multi \\
z120cm-deflection &        59.8 &   1794 &   whycode-multi \\
           z150cm &        59.7 &   1793 &   whycode-multi \\
z150cm-deflection &        59.8 &   1794 &   whycode-multi \\
           z180cm &        59.7 &   1793 &   whycode-multi \\
z180cm-deflection &        59.7 &   1793 &   whycode-multi \\
           z210cm &        59.7 &   1793 &   whycode-multi \\
z210cm-deflection &        59.7 &   1791 &   whycode-multi \\
           z240cm &        59.8 &   1794 &   whycode-multi \\
z240cm-deflection &        59.7 &   1791 &   whycode-multi \\
           z270cm &        59.7 &   1793 &   whycode-multi \\
z270cm-deflection &        59.7 &   1792 &   whycode-multi \\
           z300cm &        59.7 &   1793 &   whycode-multi \\
z300cm-deflection &        59.7 &   1791 &   whycode-multi \\
           z060cm &        59.7 &   1793 &         whycode \\
z060cm-deflection &        59.7 &   1793 &         whycode \\
           z120cm &        59.7 &   1793 &         whycode \\
z120cm-deflection &        59.7 &   1792 &         whycode \\
           z150cm &        59.7 &   1792 &         whycode \\
z150cm-deflection &        59.7 &   1791 &         whycode \\
           z180cm &        59.8 &   1794 &         whycode \\
z180cm-deflection &        59.7 &   1792 &         whycode \\
           z210cm &        59.7 &   1793 &         whycode \\
z210cm-deflection &        59.7 &   1792 &         whycode \\
           z240cm &        59.7 &   1792 &         whycode \\
z240cm-deflection &        59.8 &   1794 &         whycode \\
           z270cm &        59.8 &   1794 &         whycode \\
z270cm-deflection &        59.7 &   1793 &         whycode \\
           z300cm &        59.7 &   1793 &         whycode \\
z300cm-deflection &        59.8 &   1794 &         whycode \\
\bottomrule
\end{tabular}


==> autogenerated/test_cases.tex <==
\begin{tabular}{|lrr|rrr|rrr|rrr|}
\toprule
         Test Case & Length (s) & Frames & \multicolumn{3}{c|}{April Tag 24h10} & \multicolumn{3}{c|}{April Tag 48h12} & \multicolumn{3}{c|}{WhyCode Multi} \\
                 &          &      &             $n$ & $d$ & $r_d$ &             $n$ & $d$ & $r_d$ &           $n$ & $d$ & $r_d$ \\
\midrule
 calibration-z1.42 &     30.769 &    924 &             924 &   0 & 0.000 &             924 &   0 & 0.000 &           807 &   0 & 0.000 \\
          in-out-1 &     20.862 &    627 &             627 &  89 & 0.142 &             627 &   0 & 0.000 &           552 &  20 & 0.036 \\
          in-out-2 &     17.630 &    530 &             530 & 154 & 0.291 &             530 &   1 & 0.002 &           465 &   0 & 0.000 \\
          in-out-3 &     20.697 &    622 &             622 & 181 & 0.291 &             622 &   2 & 0.003 &           542 &   1 & 0.002 \\
          in-out-4 &     24.062 &    723 &             723 & 341 & 0.472 &             723 &  54 & 0.075 &           641 & 146 & 0.228 \\
      left-right-1 &     28.330 &    851 &             851 &   6 & 0.007 &             851 &   0 & 0.000 &           748 &  30 & 0.040 \\
      left-right-2 &     24.865 &    747 &             747 &   2 & 0.003 &             747 &   0 & 0.000 &           652 &   1 & 0.002 \\
      left-right-3 &     22.731 &    683 &             683 &   0 & 0.000 &             683 &   0 & 0.000 &           597 &   0 & 0.000 \\
      left-right-4 &     20.499 &    616 &             616 & 290 & 0.471 &             616 &  51 & 0.083 &           553 & 138 & 0.250 \\
orbit-left-right-1 &     54.567 &   1638 &            1638 &  51 & 0.031 &            1638 &   0 & 0.000 &          1424 &   2 & 0.001 \\
orbit-left-right-2 &     41.096 &   1234 &            1234 & 107 & 0.087 &            1234 &   0 & 0.000 &          1074 &   2 & 0.002 \\
orbit-left-right-3 &     56.131 &   1685 &            1685 &  72 & 0.043 &            1685 &   0 & 0.000 &          1457 &   0 & 0.000 \\
orbit-left-right-4 &     40.833 &   1226 &            1226 & 350 & 0.285 &            1226 &  33 & 0.027 &          1079 & 109 & 0.101 \\
   orbit-up-down-1 &     91.032 &   2732 &            2732 &   3 & 0.001 &            2732 &   5 & 0.002 &          2396 &   0 & 0.000 \\
   orbit-up-down-2 &     80.296 &   2410 &            2410 &   5 & 0.002 &            2410 &   1 & 0.000 &          2089 &   0 & 0.000 \\
   orbit-up-down-3 &     55.998 &   1681 &            1681 &   0 & 0.000 &            1681 &   3 & 0.002 &          1469 &   0 & 0.000 \\
   orbit-up-down-4 &     58.999 &   1771 &            1771 & 374 & 0.211 &            1771 & 138 & 0.078 &          1557 & 300 & 0.193 \\
  pan-left-right-1 &     40.398 &   1213 &            1213 &  16 & 0.013 &            1213 &   2 & 0.002 &          1066 &  24 & 0.023 \\
  pan-left-right-2 &     43.829 &   1316 &            1316 &  27 & 0.021 &            1316 &  13 & 0.010 &          1156 &  19 & 0.016 \\
  pan-left-right-3 &     39.430 &   1184 &            1184 &  16 & 0.014 &            1184 &  10 & 0.008 &          1035 &  11 & 0.011 \\
  pan-left-right-4 &     28.563 &    858 &             858 & 322 & 0.375 &             858 &  86 & 0.100 &           759 & 254 & 0.335 \\
      randomized-1 &     39.730 &   1193 &            1193 & 401 & 0.336 &            1193 &  39 & 0.033 &           991 &   5 & 0.005 \\
      randomized-2 &     24.365 &    732 &             732 & 257 & 0.351 &             732 &  16 & 0.022 &           582 &  43 & 0.074 \\
      randomized-3 &     31.199 &    937 &             937 & 381 & 0.407 &             937 &  52 & 0.055 &           718 &  44 & 0.061 \\
      randomized-4 &     36.799 &   1105 &            1105 & 460 & 0.416 &            1105 & 168 & 0.152 &           814 & 162 & 0.199 \\
    tilt-up-down-1 &     29.998 &    901 &             901 &   0 & 0.000 &             901 &   0 & 0.000 &           793 &   0 & 0.000 \\
    tilt-up-down-2 &     41.301 &   1240 &            1240 &  53 & 0.043 &            1240 &  16 & 0.013 &          1083 &  11 & 0.010 \\
    tilt-up-down-3 &     29.632 &    890 &             890 &  40 & 0.045 &             890 &  21 & 0.024 &           779 &   0 & 0.000 \\
    tilt-up-down-4 &     37.931 &   1139 &            1139 & 367 & 0.322 &            1139 & 100 & 0.088 &          1000 & 267 & 0.267 \\
         up-down-1 &     33.167 &    996 &             996 &  50 & 0.050 &             996 &   3 & 0.003 &           874 &   0 & 0.000 \\
         up-down-2 &     31.998 &    961 &             961 & 223 & 0.232 &             961 &  10 & 0.010 &           845 &   0 & 0.000 \\
         up-down-3 &     39.030 &   1172 &            1172 & 132 & 0.113 &            1172 &   1 & 0.001 &          1039 &   0 & 0.000 \\
         up-down-4 &     33.298 &   1000 &            1000 & 247 & 0.247 &            1000 &  72 & 0.072 &           883 & 233 & 0.264 \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise.tex <==
\begin{tabular}{llrrll}
\toprule
System 1 & System 2 &  $p_{=}$ &  $U_{=}$ &  $p_{\geq}$ & $U_{\geq}$ \\ \hline
\midrule
   whycode-multi &  whycode-ellipse & 0.068 &           0.0 &        &               \\ \hline
   whycode-multi &    apriltag48h12 & 0.180 &           0.0 &        &               \\ \hline
   whycode-multi &    apriltag24h10 & 0.043 &           0.0 &  0.022 &           0.0 \\ \hline
   whycode-multi &     whycode-orig & 0.043 &           0.0 &  0.022 &           0.0 \\ \hline
 whycode-ellipse &    whycode-multi & 0.068 &           0.0 &        &               \\ \hline
 whycode-ellipse &    apriltag48h12 & 0.465 &           3.0 &        &               \\ \hline
 whycode-ellipse &    apriltag24h10 & 0.043 &           0.0 &  0.022 &           0.0 \\ \hline
 whycode-ellipse &     whycode-orig & 0.043 &           0.0 &  0.022 &           0.0 \\ \hline
   apriltag48h12 &    whycode-multi & 0.180 &           0.0 &        &               \\ \hline
   apriltag48h12 &  whycode-ellipse & 0.465 &           3.0 &        &               \\ \hline
   apriltag48h12 &    apriltag24h10 & 0.043 &           0.0 &  0.022 &           0.0 \\ \hline
   apriltag48h12 &     whycode-orig & 0.080 &           1.0 &        &               \\ \hline
   apriltag24h10 &    whycode-multi & 0.043 &           0.0 &  0.978 &          15.0 \\ \hline
   apriltag24h10 &  whycode-ellipse & 0.043 &           0.0 &  0.978 &          15.0 \\ \hline
   apriltag24h10 &    apriltag48h12 & 0.043 &           0.0 &  0.978 &          15.0 \\ \hline
   apriltag24h10 &     whycode-orig & 0.686 &           6.0 &        &               \\ \hline
    whycode-orig &    whycode-multi & 0.043 &           0.0 &  0.978 &          15.0 \\ \hline
    whycode-orig &  whycode-ellipse & 0.043 &           0.0 &  0.978 &          15.0 \\ \hline
    whycode-orig &    apriltag48h12 & 0.080 &           1.0 &        &               \\ \hline
    whycode-orig &    apriltag24h10 & 0.686 &           6.0 &        &               \\ \hline
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_bundles.tex <==
\begin{tabular}{llrrrr}
\toprule
     System 1 &      System 2 &  $p_=$ & $U_=$ & $p_\geq$ & $U_\geq$ \\
\midrule
apriltag48h12 & whycode-multi &  0.117 &   145 &          &          \\
apriltag48h12 & apriltag24h10 &  0.001 &    74 &    0.000 &       74 \\
whycode-multi & apriltag48h12 &  0.117 &   145 &          &          \\
whycode-multi & apriltag24h10 &  0.007 &   101 &    0.003 &      101 \\
apriltag24h10 & apriltag48h12 &  0.001 &    74 &    1.000 &      422 \\
apriltag24h10 & whycode-multi &  0.007 &   101 &    0.997 &      364 \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_five_member.tex <==
\begin{tabular}{llrrrr}
\toprule
       System 1 &        System 2 &  $p_=$ & $U_=$ & $p_\geq$ & $U_\geq$ \\
\midrule
whycode-ellipse &   apriltag48h12 &  0.178 &   167 &          &          \\
whycode-ellipse &    whycode-orig &  0.003 &    34 &    0.001 &       34 \\
whycode-ellipse &   whycode-multi &  0.027 &   106 &    0.014 &      106 \\
whycode-ellipse &   apriltag24h10 &  0.000 &    49 &    0.000 &       49 \\
  apriltag48h12 & whycode-ellipse &  0.178 &   167 &          &          \\
  apriltag48h12 &    whycode-orig &  0.139 &   149 &          &          \\
  apriltag48h12 &   whycode-multi &  0.245 &   176 &          &          \\
  apriltag48h12 &   apriltag24h10 &  0.001 &    89 &    0.001 &       89 \\
   whycode-orig & whycode-ellipse &  0.003 &    34 &    0.999 &      219 \\
   whycode-orig &   apriltag48h12 &  0.139 &   149 &          &          \\
   whycode-orig &   whycode-multi &  0.861 &   224 &          &          \\
   whycode-orig &   apriltag24h10 &  0.008 &   123 &    0.004 &      123 \\
  whycode-multi & whycode-ellipse &  0.027 &   106 &    0.986 &      300 \\
  whycode-multi &   apriltag48h12 &  0.245 &   176 &          &          \\
  whycode-multi &    whycode-orig &  0.861 &   224 &          &          \\
  whycode-multi &   apriltag24h10 &  0.004 &   100 &    0.002 &      100 \\
  apriltag24h10 & whycode-ellipse &  0.000 &    49 &    1.000 &      447 \\
  apriltag24h10 &   apriltag48h12 &  0.001 &    89 &    0.999 &      439 \\
  apriltag24h10 &    whycode-orig &  0.008 &   123 &    0.996 &      405 \\
  apriltag24h10 &   whycode-multi &  0.004 &   100 &    0.998 &      396 \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_intra_whycode.tex <==
\begin{tabular}{llrrrr}
\toprule
       System 1 &        System 2 &  $p_=$ & $U_=$ & $p_\geq$ & $U_\geq$ \\
\midrule
  whycode-multi & whycode-ellipse &  0.003 &   116 &    0.002 &      116 \\
  whycode-multi &    whycode-orig &  0.003 &   112 &    0.001 &      112 \\
whycode-ellipse &   whycode-multi &  0.003 &   116 &    0.998 &      445 \\
whycode-ellipse &    whycode-orig &  0.514 &   244 &          &          \\
   whycode-orig &   whycode-multi &  0.003 &   112 &    0.999 &      449 \\
   whycode-orig & whycode-ellipse &  0.514 &   244 &          &          \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_single_marker.tex <==
\begin{tabular}{llrrrr}
\toprule
       System 1 &        System 2 &  $p_=$ & $U_=$ & $p_\geq$ & $U_\geq$ \\
\midrule
whycode-ellipse &   apriltag48h12 &  0.136 &   127 &          &          \\
whycode-ellipse &    whycode-orig &  0.019 &    75 &    0.009 &       75 \\
whycode-ellipse &   apriltag24h10 &  0.000 &    51 &    0.000 &       51 \\
  apriltag48h12 & whycode-ellipse &  0.136 &   127 &          &          \\
  apriltag48h12 &    whycode-orig &  0.102 &   121 &          &          \\
  apriltag48h12 &   apriltag24h10 &  0.001 &    81 &    0.001 &       81 \\
   whycode-orig & whycode-ellipse &  0.019 &    75 &    0.991 &      250 \\
   whycode-orig &   apriltag48h12 &  0.102 &   121 &          &          \\
   whycode-orig &   apriltag24h10 &  0.003 &    88 &    0.001 &       88 \\
  apriltag24h10 & whycode-ellipse &  0.000 &    51 &    1.000 &      477 \\
  apriltag24h10 &   apriltag48h12 &  0.001 &    81 &    0.999 &      415 \\
  apriltag24h10 &    whycode-orig &  0.003 &    88 &    0.999 &      377 \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_speed_bundles.tex <==
\begin{tabular}{llrrrr}
\toprule
     System 1 &      System 2 &  $p_=$ & $U_=$ & $p_\leq$ & $U_\leq$ \\
\midrule
apriltag24h10 & apriltag48h12 &  0.657 &   416 &          &          \\
apriltag24h10 & whycode-multi &  0.000 &     8 &    0.000 &        8 \\
apriltag48h12 & apriltag24h10 &  0.657 &   416 &          &          \\
apriltag48h12 & whycode-multi &  0.000 &     2 &    0.000 &        2 \\
whycode-multi & apriltag24h10 &  0.000 &     8 &    1.000 &      895 \\
whycode-multi & apriltag48h12 &  0.000 &     2 &    1.000 &      901 \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_speed_five_member.tex <==
\begin{tabular}{llrrrr}
\toprule
       System 1 &        System 2 &  $p_=$ & $U_=$ & $p_\leq$ & $U_\leq$ \\
\midrule
   whycode-orig & whycode-ellipse &  0.158 &    30 &          &          \\
   whycode-orig &   whycode-multi &  0.001 &     0 &    1.000 &      105 \\
   whycode-orig &   apriltag48h12 &  0.001 &     0 &    1.000 &      105 \\
   whycode-orig &   apriltag24h10 &  0.001 &     0 &    1.000 &      105 \\
whycode-ellipse &    whycode-orig &  0.158 &    30 &          &          \\
whycode-ellipse &   whycode-multi &  0.004 &     7 &    0.998 &       98 \\
whycode-ellipse &   apriltag48h12 &  0.001 &     0 &    1.000 &      105 \\
whycode-ellipse &   apriltag24h10 &  0.001 &     0 &    1.000 &      105 \\
  whycode-multi &    whycode-orig &  0.001 &     0 &    0.000 &        0 \\
  whycode-multi & whycode-ellipse &  0.004 &     7 &    0.002 &        7 \\
  whycode-multi &   apriltag48h12 &  0.001 &     0 &    1.000 &      105 \\
  whycode-multi &   apriltag24h10 &  0.001 &     0 &    1.000 &      105 \\
  apriltag48h12 &    whycode-orig &  0.001 &     0 &    0.000 &        0 \\
  apriltag48h12 & whycode-ellipse &  0.001 &     0 &    0.000 &        0 \\
  apriltag48h12 &   whycode-multi &  0.001 &     0 &    0.000 &        0 \\
  apriltag48h12 &   apriltag24h10 &  0.975 &    52 &          &          \\
  apriltag24h10 &    whycode-orig &  0.001 &     0 &    0.000 &        0 \\
  apriltag24h10 & whycode-ellipse &  0.001 &     0 &    0.000 &        0 \\
  apriltag24h10 &   whycode-multi &  0.001 &     0 &    0.000 &        0 \\
  apriltag24h10 &   apriltag48h12 &  0.975 &    52 &          &          \\
\bottomrule
\end{tabular}


==> autogenerated/wilcoxon_pairwise_speed_single_marker.tex <==
\begin{tabular}{llrrrr}
\toprule
       System 1 &        System 2 &  $p_=$ & $U_=$ & $p_\leq$ & $U_\leq$ \\
\midrule
  apriltag24h10 &   apriltag48h12 &  0.413 &   386 &          &          \\
  apriltag24h10 & whycode-ellipse &  0.000 &     0 &    0.000 &        0 \\
  apriltag24h10 &    whycode-orig &  0.000 &     0 &    0.000 &        0 \\
  apriltag48h12 &   apriltag24h10 &  0.413 &   386 &          &          \\
  apriltag48h12 & whycode-ellipse &  0.000 &     0 &    0.000 &        0 \\
  apriltag48h12 &    whycode-orig &  0.000 &     0 &    0.000 &        0 \\
whycode-ellipse &   apriltag24h10 &  0.000 &     0 &    1.000 &      903 \\
whycode-ellipse &   apriltag48h12 &  0.000 &     0 &    1.000 &      903 \\
whycode-ellipse &    whycode-orig &  0.008 &   241 &    0.004 &      241 \\
   whycode-orig &   apriltag24h10 &  0.000 &     0 &    1.000 &      903 \\
   whycode-orig &   apriltag48h12 &  0.000 &     0 &    1.000 &      903 \\
   whycode-orig & whycode-ellipse &  0.008 &   241 &    0.996 &      662 \\
\bottomrule
\end{tabular}


==> sections/appendices.tex <==
\subsection{Discontinuity Test Cases}
\label{appendix:discontinuity_test_cases}

Tables~\ref{table:single_marker_discontinuity_test_cases} and~\ref{table:bundle_discontinuity_test_cases} outline the
test cases for discontinuities in the single marker and bundle systems respectively.
Test cases with the same base name but different indices (e.g.~in-out-1 and in-out-2) are collected with the camera at
different distances from the fiducial marker(s), and the distance increases with the index.
These are not repeated measures.

\begin{table}[h]
    \centering
    \input{autogenerated/single_marker_discontinuity_test_cases.tex}
    \caption{The test cases for discontinuity rates of the single marker systems. $n$ is the number of detections, $d$ is the number of discontinuities, and $r_d=\frac{d}{n}$ is the discontinuity rate for each test case.}
    \label{table:single_marker_discontinuity_test_cases}
\end{table}

\begin{table}[h]
    \centering
    \input{autogenerated/bundles_discontinuity_test_cases.tex}
    \caption{The test cases for discontinuity rates of the bundle systems. $n$ is the number of detections, $d$ is the number of discontinuities, and $r_d=\frac{d}{n}$ is the discontinuity rate for each test case.}
    \label{table:bundle_discontinuity_test_cases}
\end{table}

\clearpage
\subsection{Speed Test Cases}
\label{appendix:speed_test_cases}

Tables~\ref{table:single_marker_speed_test_cases} and~\ref{table:bundle_speed_test_cases} outline the test cases for
the detection rates of the single marker and bundle systems respectively.
Test cases with the same base name but different indices (e.g.~z120cm-0 and z120cm-1) represent disjointed sections of
a longer, single video.

\begin{table}[h]
    \centering
    \input{autogenerated/single_marker_speed_test_cases.tex}
    \caption{The test cases for detection rates of the single marker systems. $\ell$ is the length in seconds of the test case, $n$ is the number of frames, $F$ is the detection rate in Hz.}
    \label{table:single_marker_speed_test_cases}
\end{table}

\begin{table}[h]
    \centering
    \input{autogenerated/bundles_speed_test_cases.tex}
    \caption{The test cases for detection rates of the bundle marker systems. $\ell$ is the length in seconds of the test case, $n$ is the number of frames, $F$ is the detection rate in Hz.}
    \label{table:bundle_speed_test_cases}
\end{table}

\clearpage
\subsection{System Parameters}
\label{appendix:system_parameters}

The folllowing section shows the runtime parameters for the fiducial systems.
For the discontinuity tests, GUI and visualization functionalities (e.g.~\texttt{image\_view}) were enabled for debugging purposes for all systems.
These were disabled during the detection rate tests to reduce extraneous computational resource usage.
We show the system parameters for our tests in Tables~\ref{table:april_tag_parameters} and~\ref{table:whycode_parameters}.
Finally, we changed the tag definitions for the April Tag systems to include a bundle of all the tags during the bundle tests,
and to include only the largest of the tags during the single marker tests.

\begin{table}[h]
    \centering
    \begin{tabular}{lr}
    \toprule
        Parameter & Value(s) \\
    \midrule
        \texttt{tag\_family} & tagCustom24h10, tagCustom48h12 \\
        \texttt{tag\_threads} & 4 \\
        \texttt{tag\_decimate} & 1.0 \\
        \texttt{tag\_blur} & 0.0 \\
        \texttt{tag\_refine\_edges} & 1 \\
        \texttt{tag\_debug} & 0 \\
        \texttt{max\_hamming\_dist} & 1 \\
        \texttt{publish\_tf} & false \\
    \bottomrule
    \end{tabular}
    \caption{The April Tag system parameters. We have changed the tag family based on which family was tested.}
    \label{table:april_tag_parameters}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{lr}
    \toprule
        Parameter & Value(s) \\
    \midrule
        \texttt{identify} & true \\
        \texttt{circleDiameter} & 0.123, 0.3 \\
        \texttt{numMarkers} & 4,3 \\
        \texttt{minSize} & 30 \\
        \texttt{fieldLength} & 1.0 \\
        \texttt{fieldWidth} & 1.0 \\
        \texttt{initialCircularityTolerance} & 100.0 \\
        \texttt{finalCircularityTolerance} & 2.0 \\
        \texttt{areaRatioTolerance} & 40.0 \\
        \texttt{centerDistanceToleranceRatio} & 10.0 \\
        \texttt{centerDistanceToleranceRatioAbs} & 5.0 \\
        \texttt{id\_bits} & 8 \\
        \texttt{id\_samples} & 360 \\
        \texttt{pub\_visual} & true, false \\
        \texttt{pub\_tf} & true, false \\
        \texttt{use\_gui} & true, false \\
    \bottomrule
    \end{tabular}
    \caption{The WhyCode system parameters. A \texttt{circleDiameter} of 0.123 corresponds to the markers in the WhyCode Multi marker, and 0.3 corresponds to the others.
    When testing for discontinuities (on a desktop) \texttt{pub\_visual}, \texttt{pub\_tf}, and \texttt{use\_gui} were set to true for visualization purposes.
    When testing for detection rate on the Raspberry Pi (in headless mode), all of these were set to false to save on computational resources.}
    \label{table:whycode_parameters}
\end{table}

%\subsection{All Figures}
%\input{autogenerated/auto_generated_appendix_figures.tex}
%
%\newpage
%\subsection{Aggregated Data}
%\input{autogenerated/auto_generated_table_all.tex}

==> sections/future_work.tex <==
%The marker systems in this paper will be further tested for autonomous precision landing on a real drone,
%where the orientation ambiguity can be destructive and a high framerate is key.
Future tests of the WhyCode Multi system could use different marker arrangements,
such as with more markers, or with the markers spaced farther apart.
All systems could be further tested
with different runtime parameters, cameras,
computational hardware, and lighting conditions.

%The marker systems in this paper will serve as a means for a drone with a monocular,
%gimbal-mounted camera to localize itself with respect to a landing pad in future studies,
%where the orientation ambiguity can be destructive and a high framerate is key.
%
%Since WhyCode is a computationally cheaper system than April Tag,
%and the WhyCode Multi method has a low discontinuity rate,
%it would be ideal to edit the WhyCode system so that markers of different sizes could be detected simultaneously.
%This would essentially allow marker embedding, in that multiple arrangements of co-planar markers could be placed
%concentrically on a single landing pad, increasing the range of view and giving it an advantage over April Tag.
%
%To make a better test of the detection rates, the ROS modules should be changed such that all systems can use the same pipeline.
%Preferably, April Tag should be edited to handle image rectification on its own.
%WhyCode could also be fed rectified images.

